Single Image Deraining with Continuous Rain Density Estimation

Single image deraining (SIDR) often suffers from over/under deraining due to the nonuniformity of rain densities and the variety of raindrop scales. In this paper, we propose a \textbf{\it co}ntinuous \textbf{\it de}nsity guided network (CODE-Net) for SIDR. Particularly, it is composed of { a rain {\color{black}streak} extractor and a denoiser}, where the convolutional sparse coding (CSC) is exploited to filter out noises from the extracted rain streaks. Inspired by the reweighted iterative soft-threshold for CSC, we address the problem of continuous rain density estimation by learning the weights with channel attention blocks from sparse codes. We further {\color{black}develop} a multiscale strategy to depict rain streaks appearing at different scales. Experiments on synthetic and real-world data demonstrate the superiority of our methods over recent {\color{black}state of the arts}, in terms of both quantitative and qualitative results. Additionally, instead of quantizing rain density with several levels, our CODE-Net can provide continuous-valued estimations of rain densities, which is more desirable in real applications.

==> extensions-1.tex <==

\begin{figure*}[!t] 
	\centering
	\begin{subfigure}[t]{0.24\linewidth}
		\includegraphics[width=1\linewidth]{extensions/gt-ext99.jpg}
		\vspace*{-0.5cm}
		\subcaption*{GT \\ (PSNR, SSIM) }
		\label{fig:ext-esrgan-gt}
	\end{subfigure}
	\hspace{-0.112cm}
	\begin{subfigure}[t]{0.24\linewidth}
		\includegraphics[width=1\linewidth]{extensions/inp-ext99.jpg}
		\vspace*{-0.5cm}
		\subcaption*{Rainy input \\ (16.67, 0.5138)}
		\label{fig:ext-esrgan-inp}
	\end{subfigure}
	\hspace{-0.112cm}
	\begin{subfigure}[t]{0.24\linewidth}
		\includegraphics[width=1\linewidth]{extensions/rdlpsnr-ext99.jpg}
		\vspace*{-0.5cm}
		\subcaption*{CODE-Net \\ (29.85, 0.8112)}
		\label{fig:ext-esrgan-psnr}
	\end{subfigure}
	\hspace{-0.112cm}
	\begin{subfigure}[t]{0.24\linewidth}
		\includegraphics[width=1\linewidth]{extensions/rdlgan-ext99.jpg}
		\vspace*{-0.5cm}
		\subcaption*{GaCODE-Net \\ (29.10, 0.8083)}
		\label{fig:ext-esrgan-gan}
	\end{subfigure}
	\caption{Visual pursuit using perceptual loss. }
	\label{fig:extesions-visual-pursuit}
\end{figure*}

==> extensions-2.tex <==
\begin{figure*}[!t] 
	\centering
	\begin{subfigure}[t]{0.49\linewidth}
		\includegraphics[width=.5\linewidth]{extensions/snow-1.jpg}\includegraphics[width=.5\linewidth]{extensions/snow-2.jpg}
		\vspace*{-0.5cm}
		\subcaption*{Snowy inputs}
	\end{subfigure}
	\hspace{-0.112cm}
	\begin{subfigure}[t]{0.49\linewidth}
		\includegraphics[width=.5\linewidth]{extensions/desnow-1.jpg}\includegraphics[width=.5\linewidth]{extensions/desnow-2.jpg}
		\vspace*{-0.5cm}
		\subcaption*{Desnowing results}
		\label{fig:snow-results}
	\end{subfigure}
	\caption{Single image  desnowing. }
	\label{fig:extesions-desnowing}
\end{figure*}

==> extensions-3.tex <==
\begin{figure*}[!t] 
	\centering
	\begin{subfigure}[t]{0.49\linewidth}
		\includegraphics[width=.65\linewidth]{extensions/10/obj-20-1.jpg}\includegraphics[width=.35\linewidth]{extensions/10/obj-20-2.png}
		\includegraphics[width=.65\linewidth]{extensions/4/obj-8-1.jpg}\includegraphics[width=.35\linewidth]{extensions/4/obj-8-2.png}
		\vspace*{-0.5cm}
		\subcaption*{Rainy inputs}
	\end{subfigure}
	\hspace{-0.112cm}
	\begin{subfigure}[t]{0.49\linewidth}
		\includegraphics[width=.65\linewidth]{extensions/10/obj-19-1.jpg}\includegraphics[width=.35\linewidth]{extensions/10/obj-19-2.png}
		\includegraphics[width=.65\linewidth]{extensions/4/obj-7-1.jpg}\includegraphics[width=.35\linewidth]{extensions/4/obj-7-2.png}
		\vspace*{-0.5cm}
		\subcaption*{Deraining results}
	\end{subfigure}
	\caption{Object detection with/without deraining. }
	\label{fig:extesions-google-api-1}
\end{figure*}

==> extensions.tex <==

\begin{figure*}[!t] 
	\centering
	\begin{subfigure}[t]{0.24\linewidth}
		\includegraphics[width=1\linewidth]{extensions/gt-ext99.jpg}
		\vspace*{-0.5cm}
		\subcaption*{GT \\ (PSNR,SSIM) }
		\label{fig:ext-esrgan-gt}
	\end{subfigure}
	\hspace{-0.112cm}
	\begin{subfigure}[t]{0.24\linewidth}
		\includegraphics[width=1\linewidth]{extensions/inp-ext99.jpg}
		\vspace*{-0.5cm}
		\subcaption*{Rainy input \\ (16.67,0.5138)}
		\label{fig:ext-esrgan-inp}
	\end{subfigure}
	\hspace{-0.112cm}
	\begin{subfigure}[t]{0.24\linewidth}
		\includegraphics[width=1\linewidth]{extensions/rdlpsnr-ext99.jpg}
		\vspace*{-0.5cm}
		\subcaption*{RDL \\ (29.85,0.8112)}
		\label{fig:ext-esrgan-psnr}
	\end{subfigure}
	\hspace{-0.112cm}
	\begin{subfigure}[t]{0.24\linewidth}
		\includegraphics[width=1\linewidth]{extensions/rdlgan-ext99.jpg}
		\vspace*{-0.5cm}
		\subcaption*{GaRDL \\ (29.10,0.8083)}
		\label{fig:ext-esrgan-gan}
	\end{subfigure}
	\caption{Extension: visual pursuit using perceptual loss }
	\label{fig:extesions-visual-pursuit}
\end{figure*}

\begin{figure*}[!t] 
	\centering
	\begin{subfigure}[t]{0.49\linewidth}
		\includegraphics[width=.5\linewidth]{extensions/snow-1.jpg}\includegraphics[width=.5\linewidth]{extensions/snow-2.jpg}
		\vspace*{-0.5cm}
		\subcaption*{Snowy inputs}
	\end{subfigure}
	\hspace{-0.112cm}
	\begin{subfigure}[t]{0.49\linewidth}
		\includegraphics[width=.5\linewidth]{extensions/desnow-1.jpg}\includegraphics[width=.5\linewidth]{extensions/desnow-2.jpg}
		\vspace*{-0.5cm}
		\subcaption*{Desnowing results}
		\label{fig:snow-results}
	\end{subfigure}
	\caption{Extension: single image  desnowing. }
	\label{fig:extesions-desnowing}
\end{figure*}

==> result2.tex <==

\begin{figure*}[!t]
	\centering
	\begin{subfigure}[t]{0.2\linewidth}
		\includegraphics[width=1.\linewidth]{results/real1-inp-wds.pdf} %inp
		\vspace*{-0.5cm}
		\subcaption*{Input}
	\end{subfigure}
	\hspace{-0.12cm}
	\begin{subfigure}[t]{0.2\linewidth}
		\includegraphics[width=1.\linewidth]{results/real1-gmm-wds.pdf} %gmm
		\vspace*{-0.5cm}
		\subcaption*{GMM \cite{gmm}}
	\end{subfigure}
	\hspace{-0.12cm}
	\begin{subfigure}[t]{0.2\linewidth} 
		\includegraphics[width=1.\linewidth]{results/real1-cnn-wds.pdf}  %cnn
		\vspace*{-0.5cm}
		\subcaption*{CNN \cite{cnn}}
	\end{subfigure} 
	\hspace{-0.12cm}
	\begin{subfigure}[t]{0.2\linewidth}
		\includegraphics[width=1.\linewidth]{results/real1-ddn-wds.pdf}  %ddn
		\vspace*{-0.5cm}
		\subcaption*{DDN \cite{ddn}}
	\end{subfigure}
	\hspace{-0.12cm}
	\begin{subfigure}[t]{0.2\linewidth}
		\includegraphics[width=1.\linewidth]{results/real1-jorder-wds.pdf}  %jorder
		\vspace*{-0.5cm}
		\subcaption*{JORDER \cite{jorder}}
	\end{subfigure}
	\hspace{-0.12cm}
	\begin{subfigure}[t]{0.2\linewidth}
		\includegraphics[width=1.\linewidth]{results/real1-didmdn-wds.pdf}  %didmdn
		\vspace*{-0.5cm}
		\subcaption*{DID-MDN \cite{did-mdn}}
	\end{subfigure}
	\hspace{-0.12cm}
	\begin{subfigure}[t]{0.2\linewidth}
		\includegraphics[width=1.\linewidth]{results/real1-rdl-wds.pdf}  %rdl
		\vspace*{-0.4cm}
		\subcaption*{RDL(ours)}
	\end{subfigure}
	\hspace{-0.12cm}
	\begin{subfigure}[t]{0.2\linewidth}
		\includegraphics[width=1.\linewidth]{results/real1-mrdl-wds.pdf}  %mrdl
		\vspace*{-0.4cm}
		\subcaption*{mRDL(ours)}
	\end{subfigure}\\	
	\centering
	\begin{subfigure}[t]{0.2\linewidth}
		\includegraphics[width=1.\linewidth]{results/real4-inp-wds.pdf}
		\vspace*{-0.5cm}
							\subcaption*{Input}
	\end{subfigure}
	\hspace{-0.112cm}
	\begin{subfigure}[t]{0.2\linewidth}
		\includegraphics[width=1.\linewidth]{results/real4-gmm-wds.pdf}
		\vspace*{-0.5cm}
							\subcaption*{GMM \cite{gmm}}
	\end{subfigure}
	\hspace{-0.112cm}
	\begin{subfigure}[t]{0.2\linewidth}
		\includegraphics[width=1.\linewidth]{results/real4-cnn-wds.pdf}
		\vspace*{-0.5cm}
							\subcaption*{CNN \cite{cnn}}
	\end{subfigure} 
	\hspace{-0.112cm}
	\begin{subfigure}[t]{0.2\linewidth}
		\includegraphics[width=1.\linewidth]{results/real4-ddn-wds.pdf}
		\vspace*{-0.5cm}
							\subcaption*{DDN \cite{ddn}}
	\end{subfigure}
	\hspace{-0.112cm}
	\begin{subfigure}[t]{0.2\linewidth}
		\includegraphics[width=1.\linewidth]{results/real4-jorder-wds.pdf}
		\vspace*{-0.5cm}
							\subcaption*{JORDER \cite{jorder}}
	\end{subfigure}
	\hspace{-0.112cm}
	\begin{subfigure}[t]{0.2\linewidth}
		\includegraphics[width=1.\linewidth]{results/real4-didmdn-wds.pdf}
		\vspace*{-0.5cm}
							\subcaption*{ DID-MDN \cite{did-mdn}}
	\end{subfigure}
	\hspace{-0.112cm}
	\begin{subfigure}[t]{0.2\linewidth}
		\includegraphics[width=1.\linewidth]{results/real4-rdl-wds.pdf}
		\vspace*{-0.5cm}
		\subcaption*{RDL(ours)}
	\end{subfigure}
	\hspace{-0.112cm}
	\begin{subfigure}[t]{0.2\linewidth}
		\includegraphics[width=1.\linewidth]{results/real4-mrdl-wds.pdf}
		\vspace*{-0.5cm}
		\subcaption*{mRDL(ours)}
	\end{subfigure}

	\caption{Qualitative comparisons of two real images.}
	\label{Qualitative_comparison_on_real}
\end{figure*}

==> result4.tex <==

\begin{figure*}[!t]
	\centering
	\begin{subfigure}[t]{0.2\linewidth}
		\includegraphics[width=1.\linewidth]{final-results/inp/43.jpg} %inp
		\vspace*{-0.5cm}
		\subcaption*{Input}
	\end{subfigure}
	\hspace{-0.12cm}
	\begin{subfigure}[t]{0.2\linewidth}
		\includegraphics[width=1.\linewidth]{final-results/ddn/43.jpg} %ddn
		\vspace*{-0.5cm}
		\subcaption*{DDN \cite{ddn}}
	\end{subfigure}
	\hspace{-0.12cm}
	\begin{subfigure}[t]{0.2\linewidth} 
		\includegraphics[width=1.\linewidth]{final-results/didmdn/9_GT.jpg}  %didmdn
		\vspace*{-0.5cm}
		\subcaption*{DID-MDN \cite{did-mdn}}
	\end{subfigure} 
	\hspace{-0.12cm}
	\begin{subfigure}[t]{0.2\linewidth}
		\includegraphics[width=1.\linewidth]{final-results/semi/43_out.jpg}  %semi
		\vspace*{-0.5cm}
		\subcaption*{SEMI \cite{semi}}
	\end{subfigure}
	\hspace{-0.12cm}
	\begin{subfigure}[t]{0.2\linewidth}
		\includegraphics[width=1.\linewidth]{final-results/spanet/97.jpg}  %spanet
		\vspace*{-0.5cm}
		\subcaption*{SPANet \cite{spanet}}
	\end{subfigure}
	\hspace{-0.12cm}
	\begin{subfigure}[t]{0.2\linewidth}
		\includegraphics[width=1.\linewidth]{final-results/prenet/43.jpg}  %prenet
		\vspace*{-0.5cm}
		\subcaption*{PreNet \cite{prenet}}
	\end{subfigure}
	\hspace{-0.12cm}
	\begin{subfigure}[t]{0.2\linewidth}
		\includegraphics[width=1.\linewidth]{final-results/rdl/ftd10000-43.jpg}  %rdl
		\vspace*{-0.4cm}
		\subcaption*{RDL(ours)}
	\end{subfigure}
	\hspace{-0.12cm}
	\begin{subfigure}[t]{0.2\linewidth}
		\includegraphics[width=1.\linewidth]{final-results/mrdl/43.jpg}  %mrdl
		\vspace*{-0.4cm}
		\subcaption*{mRDL(ours)}
	\end{subfigure}\\	
	\centering
	\begin{subfigure}[t]{0.2\linewidth}
		\includegraphics[width=1.\linewidth]{final-results/inp/66.jpg} %inp
		\vspace*{-0.5cm}
		\subcaption*{Input}
	\end{subfigure}
	\hspace{-0.12cm}
	\begin{subfigure}[t]{0.2\linewidth}
		\includegraphics[width=1.\linewidth]{final-results/ddn/inp_66.jpg} %ddn
		\vspace*{-0.5cm}
		\subcaption*{DDN \cite{ddn}}
	\end{subfigure}
	\hspace{-0.12cm}
	\begin{subfigure}[t]{0.2\linewidth} 
		\includegraphics[width=1.\linewidth]{final-results/didmdn/5_GT.jpg}  %didmdn
		\vspace*{-0.5cm}
		\subcaption*{DID-MDN \cite{did-mdn}}
	\end{subfigure} 
	\hspace{-0.12cm}
	\begin{subfigure}[t]{0.2\linewidth}
		\includegraphics[width=1.\linewidth]{final-results/semi/66_out.jpg}  %semi
		\vspace*{-0.5cm}
		\subcaption*{SEMI \cite{semi}}
	\end{subfigure}
	\hspace{-0.12cm}
	\begin{subfigure}[t]{0.2\linewidth}
		\includegraphics[width=1.\linewidth]{final-results/spanet/28.jpg}  %spanet
		\vspace*{-0.5cm}
		\subcaption*{SPANet \cite{spanet}}
	\end{subfigure}
	\hspace{-0.12cm}
	\begin{subfigure}[t]{0.2\linewidth}
		\includegraphics[width=1.\linewidth]{final-results/prenet/inp_66.jpg}  %prenet
		\vspace*{-0.5cm}
		\subcaption*{PreNet \cite{prenet}}
	\end{subfigure}
	\hspace{-0.12cm}
	\begin{subfigure}[t]{0.2\linewidth}
		\includegraphics[width=1.\linewidth]{final-results/rdl/inp_66.jpg}  %rdl
		\vspace*{-0.4cm}
		\subcaption*{RDL(ours)}
	\end{subfigure}
	\hspace{-0.12cm}
	\begin{subfigure}[t]{0.2\linewidth}
		\includegraphics[width=1.\linewidth]{final-results/mrdl/inp_66.jpg}  %mrdl
		\vspace*{-0.4cm}
		\subcaption*{mRDL(ours)}
	\end{subfigure}
	\caption{Qualitative comparisons of two real images.}
	\label{Qualitative_comparison_on_real}
\end{figure*}

==> result5-rde.tex <==
\begin{figure*}[!t]
	\centering
	\begin{subfigure}[t]{0.2\linewidth}
		\includegraphics[width=1.\linewidth]{final-results/inp/43.jpg} %inp
		\vspace*{-0.5cm}
		\subcaption*{Input \\ 0.0183}
	\end{subfigure}
	\hspace{-0.12cm}
	\begin{subfigure}[t]{0.2\linewidth}
		\includegraphics[width=1.\linewidth]{final-results/ddn/43.jpg} %ddn
		\vspace*{-0.5cm}
		\subcaption*{DDN \cite{ddn} \\ 0.0067}
	\end{subfigure}
	\hspace{-0.12cm}
	\begin{subfigure}[t]{0.2\linewidth} 
		\includegraphics[width=1.\linewidth]{final-results/didmdn/9_GT.jpg}  %didmdn
		\vspace*{-0.5cm}
		\subcaption*{DID-MDN \cite{did-mdn} \\0.0250}
	\end{subfigure} 
	\hspace{-0.12cm}
	\begin{subfigure}[t]{0.2\linewidth}
		\includegraphics[width=1.\linewidth]{final-results/semi/43_out.jpg}  %semi
		\vspace*{-0.5cm}
		\subcaption*{SEMI \cite{semi} \\ 0.0083}
	\end{subfigure}
	\hspace{-0.12cm}
	\begin{subfigure}[t]{0.2\linewidth}
		\includegraphics[width=1.\linewidth]{final-results/spanet/97.jpg}  %spanet
		\vspace*{-0.5cm}
		\subcaption*{SPANet \cite{spanet} \\0.0066}
	\end{subfigure}
	\hspace{-0.12cm}
	\begin{subfigure}[t]{0.2\linewidth}
		\includegraphics[width=1.\linewidth]{final-results/prenet/43.jpg}  %prenet
		\vspace*{-0.5cm}
		\subcaption*{PreNet \cite{prenet} \\0.0133}
	\end{subfigure}
	\hspace{-0.12cm}
	\begin{subfigure}[t]{0.2\linewidth}
		\includegraphics[width=1.\linewidth]{final-results/rdl/ftd10000-43.jpg}  %rdl
		\vspace*{-0.4cm}
		\subcaption*{CODE-Net (ours) \\0.0150}
	\end{subfigure}
	\hspace{-0.12cm}
	\begin{subfigure}[t]{0.2\linewidth}
		\includegraphics[width=1.\linewidth]{final-results/mrdl/43.jpg}  %mrdl
		\vspace*{-0.4cm}
		\subcaption*{mCODE-Net (ours) \\0.0100}
	\end{subfigure}\\	
	\centering
	\begin{subfigure}[t]{0.2\linewidth}
		\includegraphics[width=1.\linewidth]{final-results/inp/130.jpg} %inp
		\vspace*{-0.5cm}
		\subcaption*{Input \\0.3233}
	\end{subfigure}
	\hspace{-0.12cm}
	\begin{subfigure}[t]{0.2\linewidth}
		\includegraphics[width=1.\linewidth]{final-results/ddn/130.jpg} %ddn
		\vspace*{-0.5cm}
		\subcaption*{DDN \cite{ddn} \\0.1617}
	\end{subfigure}
	\hspace{-0.12cm}
	\begin{subfigure}[t]{0.2\linewidth} 
		\includegraphics[width=1.\linewidth]{final-results/didmdn/10_GT.jpg}  %didmdn
		\vspace*{-0.5cm}
		\subcaption*{DID-MDN \cite{did-mdn} \\0.1600}
	\end{subfigure} 
	\hspace{-0.12cm}
	\begin{subfigure}[t]{0.2\linewidth}
		\includegraphics[width=1.\linewidth]{final-results/semi/130_out.jpg}  %semi
		\vspace*{-0.5cm}
		\subcaption*{SEMI \cite{semi} \\0.2950}
	\end{subfigure}
	\hspace{-0.12cm}
	\begin{subfigure}[t]{0.2\linewidth}
		\includegraphics[width=1.\linewidth]{final-results/spanet/89.jpg}  %spanet
		\vspace*{-0.5cm}
		\subcaption*{SPANet \cite{spanet} \\0.1183}
	\end{subfigure}
	\hspace{-0.12cm}
	\begin{subfigure}[t]{0.2\linewidth}
		\includegraphics[width=1.\linewidth]{final-results/prenet/130.jpg}  %prenet
		\vspace*{-0.5cm}
		\subcaption*{PreNet \cite{prenet} \\ 0.1000}
	\end{subfigure}
	\hspace{-0.12cm}
	\begin{subfigure}[t]{0.2\linewidth}
		\includegraphics[width=1.\linewidth]{final-results/rdl/ftd10000-130.jpg}  %rdl
		\vspace*{-0.4cm}
		\subcaption*{CODE-Net (ours) \\ 0.1433}
	\end{subfigure}
	\hspace{-0.12cm}
	\begin{subfigure}[t]{0.2\linewidth}
		\includegraphics[width=1.\linewidth]{final-results/mrdl/130.jpg}  %mrdl
		\vspace*{-0.4cm}
		\subcaption*{mCODE-Net (ours) \\0.1517}
	\end{subfigure}
	\caption{Qualitative comparisons of two real images with light rain and the corresponding RDEs are calculated by \myref{rain-density-estimation}.}
	\label{Qualitative_comparison_on_real1}
\end{figure*}

==> result5.tex <==

\begin{figure*}[!t]
	\centering
	\begin{subfigure}[t]{0.2\linewidth}
		\includegraphics[width=1.\linewidth,trim=0 127 0 0 ,clip]{final-results/inp/56.jpg} %inp
		\vspace*{-0.5cm}
		\subcaption*{Input}
	\end{subfigure}
	\hspace{-0.12cm}
	\begin{subfigure}[t]{0.2\linewidth}
		\includegraphics[width=1.\linewidth,trim=0 127 0 0 ,clip]{final-results/ddn/56.jpg} %ddn
		\vspace*{-0.5cm}
		\subcaption*{DDN \cite{ddn}}
	\end{subfigure}
	\hspace{-0.12cm}
	\begin{subfigure}[t]{0.2\linewidth} 
		\includegraphics[width=1.\linewidth,trim=0 127 0 0 ,clip]{final-results/didmdn/1_GT.jpg}  %didmdn
		\vspace*{-0.5cm}
		\subcaption*{DID-MDN \cite{did-mdn}}
	\end{subfigure} 
	\hspace{-0.12cm}
	\begin{subfigure}[t]{0.2\linewidth}
		\includegraphics[width=1.\linewidth,trim=0 127 0 0 ,clip]{final-results/semi/56_out.jpg}  %semi
		\vspace*{-0.5cm}
		\subcaption*{SEMI \cite{semi}}
	\end{subfigure}
	\hspace{-0.12cm}
	\begin{subfigure}[t]{0.2\linewidth}
		\includegraphics[width=1.\linewidth]{final-results/spanet/new95.jpg}  %spanet
		\vspace*{-0.5cm}
		\subcaption*{SPANet \cite{spanet}}
	\end{subfigure}
	\hspace{-0.12cm}
	\begin{subfigure}[t]{0.2\linewidth}
		\includegraphics[width=1.\linewidth,trim=0 127 0 0 ,clip]{final-results/prenet/56.jpg}  %prenet
		\vspace*{-0.5cm}
		\subcaption*{PreNet \cite{prenet}}
	\end{subfigure}
	\hspace{-0.12cm}
	\begin{subfigure}[t]{0.2\linewidth}
		\includegraphics[width=1.\linewidth,trim=0 127 0 0 ,clip]{final-results/rdl/ftd10000-56.jpg}  %rdl
		\vspace*{-0.4cm}
		\subcaption*{RDL(ours)}
	\end{subfigure}
	\hspace{-0.12cm}
	\begin{subfigure}[t]{0.2\linewidth}
		\includegraphics[width=1.\linewidth,trim=0 127 0 0 ,clip]{final-results/mrdl/56.jpg}  %mrdl
		\vspace*{-0.4cm}
		\subcaption*{mRDL(ours)}
	\end{subfigure}\\	
	\centering
	\begin{subfigure}[t]{0.2\linewidth}
		\includegraphics[width=1.\linewidth]{final-results/inp/130.jpg} %inp
		\vspace*{-0.5cm}
		\subcaption*{Input}
	\end{subfigure}
	\hspace{-0.12cm}
	\begin{subfigure}[t]{0.2\linewidth}
		\includegraphics[width=1.\linewidth]{final-results/ddn/130.jpg} %ddn
		\vspace*{-0.5cm}
		\subcaption*{DDN \cite{ddn}}
	\end{subfigure}
	\hspace{-0.12cm}
	\begin{subfigure}[t]{0.2\linewidth} 
		\includegraphics[width=1.\linewidth]{final-results/didmdn/10_GT.jpg}  %didmdn
		\vspace*{-0.5cm}
		\subcaption*{DID-MDN \cite{did-mdn}}
	\end{subfigure} 
	\hspace{-0.12cm}
	\begin{subfigure}[t]{0.2\linewidth}
		\includegraphics[width=1.\linewidth]{final-results/semi/130_out.jpg}  %semi
		\vspace*{-0.5cm}
		\subcaption*{SEMI \cite{semi}}
	\end{subfigure}
	\hspace{-0.12cm}
	\begin{subfigure}[t]{0.2\linewidth}
		\includegraphics[width=1.\linewidth]{final-results/spanet/89.jpg}  %spanet
		\vspace*{-0.5cm}
		\subcaption*{SPANet \cite{spanet}}
	\end{subfigure}
	\hspace{-0.12cm}
	\begin{subfigure}[t]{0.2\linewidth}
		\includegraphics[width=1.\linewidth]{final-results/prenet/130.jpg}  %prenet
		\vspace*{-0.5cm}
		\subcaption*{PreNet \cite{prenet}}
	\end{subfigure}
	\hspace{-0.12cm}
	\begin{subfigure}[t]{0.2\linewidth}
		\includegraphics[width=1.\linewidth]{final-results/rdl/ftd10000-130.jpg}  %rdl
		\vspace*{-0.4cm}
		\subcaption*{RDL(ours)}
	\end{subfigure}
	\hspace{-0.12cm}
	\begin{subfigure}[t]{0.2\linewidth}
		\includegraphics[width=1.\linewidth]{final-results/mrdl/130.jpg}  %mrdl
		\vspace*{-0.4cm}
		\subcaption*{mRDL(ours)}
	\end{subfigure}
	\caption{Qualitative comparisons of two real images.}
	\label{Qualitative_comparison_on_real1}
\end{figure*}

==> results_real.tex <==
\begin{figure}[!t] 
	\centering
	\begin{subfigure}[t]{0.32\linewidth}
		\includegraphics[width=1.\linewidth]{results_real/a-norm.pdf}
		\includegraphics[width=1.\linewidth]{results_real/spanet-48}
		\includegraphics[width=1.\linewidth]{results_real/a-derain-norm.pdf}
%		\vspace*{-0.3cm}
		\subcaption{ light }
	\end{subfigure}
	\begin{subfigure}[t]{0.32\linewidth}
		\includegraphics[width=1.\linewidth]{results_real/d-norm.pdf}
		\includegraphics[width=1.\linewidth]{results_real/spanet-44}
		\includegraphics[width=1.\linewidth]{results_real/d-derain-norm.pdf}
%		\vspace*{-0.3cm}
		\subcaption{medium}
	\end{subfigure}
	\begin{subfigure}[t]{0.32\linewidth}
		\includegraphics[width=1.\linewidth]{results_real/c-norm.pdf}
		\includegraphics[width=1.\linewidth]{results_real/spanet-42}
		\includegraphics[width=1.\linewidth]{results_real/c-derain-norm.pdf}
%		\vspace*{-0.3cm}
		\subcaption{heavy  }
	\end{subfigure} 
	\caption{Real deraining results on light, medium and heavy rain of our model, with the density estimation in the bottom (yellow: rainy inputs; blue: deraining results). }
	\label{fig:1-real}
	\vspace{-0.2cm}
\end{figure}


==> runtime.tex <==
{	
	\begin{table*}[!t]  
		\centering  
		\fontsize{6.5}{8}\selectfont  
		\begin{threeparttable}  
			\caption{Running time (in seconds) for different methods averaged
				on 100 images with size 512 $ \times $ 512. `*' indicates that the method is tested on CPU.} 
			
			\label{tab:runtime}
			\begin{tabular}{cccccccccccc}
				\toprule     
				Method&DSC*\cite{dsc}&GMM*\cite{gmm}&CNN~\cite{cnn}&DDN~\cite{ddn}&JORDER~\cite{jorder}&DID-MDN~\cite{did-mdn}& PreNet~\cite{prenet}&SPANet~\cite{spanet}&SEMI~\cite{semi}&DenNet (ours)&mDenNet (ours)\cr  
				\midrule 
				Time(s)&124.369&$\geq$650&0.603&0.319&0.110&0.230& 0.151&0.353&0.483&  0.328&0.833\cr				
				\bottomrule  
			\end{tabular} 

		\end{threeparttable}  
	\end{table*}  
}
%&mRDL(ours)
%&0.833

==> tab_vis_comparison.tex <==
\begin{table}[!t]  
		\centering  
		\fontsize{7.5}{9}\selectfont  
		\begin{threeparttable}  
			\caption{Average PSNR/SSIMs on Rain12, Rain1200 and Test1000.  \textbf{Bold}: the best; \underline{underline}: the second best.} 
			
			\label{tab:performance_comparison}
			\begin{tabular}{cccccccccc}
				\toprule  
				\multirow{2}{*}{\makecell{Methods\\[-.19cm]}}& 
				\multicolumn{2}{c}{Rain12}&\multicolumn{2}{c}{Rain1200}&\multicolumn{2}{c}{Test1000}\cr  
				\cmidrule(lr){2-3} \cmidrule(lr){4-5}\cmidrule(lr){6-7}      
				&PSNR&SSIM&PSNR&SSIM&PSNR&SSIM\cr  
				\midrule 
				
				%Input&30.14&0.8553&4.645&23.63&0.7324&3.190\cr  
				DSC~\cite{dsc}  &29.98&0.8654  &21.44&0.7896&32.33&0.9305\cr  
				GMM~\cite{gmm} &32.15&0.9145&22.75&0.8352&32.99&0.9475\cr 
				CNN~\cite{cnn}   &33.33&0.9199&23.55&0.8352&31.31&0.9304\cr
				JORDER~\cite{jorder}   & {36.15}&0.9548&25.71&0.8074&35.72&{0.9776}\cr
				DDN~\cite{ddn}   & 29.84&0.9049& 30.08&0.8791&34.88&0.9727\cr 
				DID-MDN~\cite{did-mdn} &29.49 &0.9031&29.65&0.9016&28.96&0.9457\cr
				%SEMI\cite{semi} &- &-&26.05&0.8220&-&-\cr
				PreNet~\cite{prenet} & \underline{36.66} &0.9610&30.56&0.8750&30.31&0.9538\cr
				SPANet~\cite{spanet} &32.71 &0.9285&30.05&\bf 0.9342&38.53& \underline{0.9875}\cr
				\midrule
				CODE-Net~(ours) &{ 36.21}&\underline{ 0.9618}&{ \underline {33.31} }&{ {0.9174}}&\underline{ 38.88}&0.9867\cr
				mCODE-Net~(ours)  &\bf { 36.79}&{ \bf {0.9639}}&{\bf {34.03}}&\underline{ 0.9281}&{\bf 39.85}&\bf 0.9879\cr  				
				\bottomrule  
			\end{tabular} 
			
		\end{threeparttable}  
	\end{table}  

==> tab_vis_comparison_runtime.tex <==
\begin{table}[!t]  
		\centering  
		\fontsize{7.2}{9}\selectfont  
		\begin{threeparttable}  
			\caption{Average PSNR/SSIMs on Rain12, Rain1200 and Test1000. Average running time (second) on 100 images with size 512 $ \times $ 512. `*' indicates that the method is tested on CPU.} 
			
			\label{tab:performance_comparison}
			\begin{tabular}{p{1.6cm}<{\centering}p{1.4cm}<{\centering}p{1.4cm}<{\centering}p{1.4cm}<{\centering}p{0.8cm}<{\centering}}
				\toprule  
				\multirow{2}{*}{\makecell{Methods\\[-.15cm]}}& 
				\multicolumn{1}{c}{Rain12}&\multicolumn{1}{c}{Rain1200}&\multicolumn{1}{c}{Test1000}&\multicolumn{1}{c}{512$\times$512}\cr  
				\cmidrule(lr){2-2} \cmidrule(lr){3-3}\cmidrule(lr){4-4}    \cmidrule(lr){5-5}  
				&PSNR/SSIM&PSNR/SSIM&PSNR/SSIM&Time\cr  
				\midrule 
				
				%Input&30.14&0.8553&4.645&23.63&0.7324&3.190\cr  
				DSC*\cite{dsc}  &29.98/0.8654  &21.44/0.7896&32.33/0.9305&124.369\cr  
				GMM*\cite{gmm} &32.15/0.9145&22.75/0.8352&32.99/0.9475&$\geq$650\cr 
				CNN~\cite{cnn}   &33.33/0.9199&23.55/0.8352&31.31/0.9304&0.603\cr
				JORDER~\cite{jorder}   & {36.15}/0.9548&25.71/0.8074&35.72/{0.9776}&\bf 0.110\cr
				DDN~\cite{ddn}   & 29.84/0.9049& 30.08/0.8791&34.88/0.9727&0.319\cr 
				DID-MDN~\cite{did-mdn} &29.49 /0.9031&29.65/0.9016&28.96/0.9457&0.230\cr
				%SEMI\cite{semi} &- &-&26.05&0.8220&-&-\cr
				PreNet~\cite{prenet} & \underline{36.66} /0.9610&30.56/0.8750&30.31/0.9538&\underline{0.151}\cr
				SPANet~\cite{spanet} &32.71 /0.9285&30.05/\bf 0.9342&38.53/ \underline{0.9875}&0.353\cr
				\midrule
				CODE-Net &{ 36.21}/\underline{ 0.9618}&{ \underline {33.31} }/0.9174&\underline{ 38.88}/0.9867&0.328\cr
				mCODE-Net  &\bf { 36.79}/{ \bf {0.9639}}&{\bf {34.03}}/\underline{ 0.9281}&{\bf 39.85}/\bf 0.9879&0.833\cr  				
				\bottomrule  
			\end{tabular} 
			
		\end{threeparttable}  
	\end{table}  
